Optimization of Energy Harvesting MISO Communication System with Feedback

Optimization of a point-to-point (p2p) multipleinput single-output (MISO) communication system is considered when both the transmitter (TX) and the receiver (RX) have energy harvesting (EH) capabilities. The RX is interested in feeding back the channel state information (CSI) to the TX to help improve the transmission rate. The objective is to maximize the throughput by a deadline, subject to the EH constraints at the TX and the RX. The throughput metric considered is an upper bound on the ergodic rate of the MISO channel with beamforming and limited feedback. Feedback bit allocation and transmission policies that maximize the upper bound on the ergodic rate are obtained. Tools from majorization theory are used to simplify the formulated optimization problems. Optimal policies obtained for the modified problem outperform the naive scheme in which no intelligent management of energy is performed.

==> library/math_lib.tex <==

\usepackage{bm,cite}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{amsbsy}
\usepackage{latexsym}
\usepackage{amssymb}
\usepackage{wasysym}


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{remark}{Remark}




\DeclareMathAlphabet{\mathbit}{OML}{cmr}{bx}{it}
\DeclareMathAlphabet{\mathsf}{OT1}{cmss}{m}{n}
\DeclareMathAlphabet{\mathTXf}{OT1}{cmss}{bx}{it}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\nondiag}{nondiag}
\DeclareMathOperator{\blockdiag}{blockdiag}
\DeclareMathOperator{\trace}{tr}
\DeclareMathOperator{\nullsp}{null}
\DeclareMathOperator{\vectorize}{vec}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\Bild}{bild}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\imj}{j}
\DeclareMathOperator{\Transpose}{T}
\DeclareMathOperator{\h}{\phi}
\DeclareMathOperator{\daggerrmitian}{H}
%\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmax}{arg\ max}
%\DeclareMathOperator*{\min}{min}
%\DeclareMathOperator*{\max}{max}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator{\Real}{Re}
\DeclareMathOperator{\Imag}{Im}
\DeclareMathOperator{\Exp}{E}
\DeclareMathOperator{\SINR}{SINR}
\DeclareMathOperator{\SNR}{SNR}
\DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}


% Zur Notation von Zufallsgroessen ohne Serifen
\newcommand{\TX}{\mathbit}
\newcommand{\bcal}[1]{\boldsymbol{\cal #1}}
\newcommand{\brandom}{\mathTXf}
\newcommand{\intd}{{\,\operatorname{d}}}
\newcommand{\diffd}{{\operatorname{d}}}
\newcommand{\e}{{\operatorname{e}}}
%\newcommand{\E}[1]{{\operatorname{E}\left[#1\right]}}
\newcommand{\CC}[1]{\B{C}_{#1}} %for covariance matrices
\newcommand{\I}{\mathbf{I}} %identity matrix
\newcommand{\Z}{\mathbf{0}} %null vector or null matrix
\newcommand{\U}{\mathbf{1}} %all-ones vector or all-ones matrix
\newcommand{\norm}[1]{\lVert{#1}\rVert}
\newcommand{\Sum}{{\text{sum}}}
\newcommand{\Comp}{{\text{comp}}}
\newcommand{\Tx}{{\text{Tx}}}
%\newcommand{\dagger}{{\text{H}}}
\newcommand{\Approx}{{\text{approx}}}
\newcommand{\FM}{{\text{FM}}}
\newcommand{\Up}{{\text{up}}}
\newcommand{\Low}{{\text{low}}}
\newcommand{\Maj}{{\text{Maj}}}
\newcommand{\Min}{{\text{Min}}}
\newcommand{\BF}{{\text{BF}}}
\newcommand{\Tr}{{\Transpose}}
\newcommand{\Fro}{{\text{F}}}
\newcommand{\Int}{{\text{Int}}}
\newcommand{\tr}{{\text{tr}}}
\newcommand{\Eq}{{\text{Equality}}}
\newcommand{\as}{{\text{asympt}}}
\newcommand{\PTP}{{\text{PTP}}}
\newcommand{\virt}{{\text{v}}}
\newcommand{\MG}{{\text{M}_{\text{G}}}}
\newcommand{\MGF}{{{\text{MGF}}}}
%\newcommand{\VdM}{{\tau}}
\newcommand{\sign}{{{\text{sign}}}} 
\newcommand{\opt}{{{\text{opt}}}} 
\newcommand{\proj}{{{\bot}}}  
\newcommand{\RO}{{\text{R}_{\text{O}}}}

\newcommand{\E}{{\text{E}}}
\newcommand{\Snr}{{\text{Snr}}}
\newcommand{\inst}{{\text{Inst}}}
\newcommand{\MMSE}{{\text{MMSE}}} 
\newcommand{\trans}{{\text{T}}} 
\newcommand{\rec}{{\text{R}}} 
\newcommand{\He}{{{\text{H}}}} 
\newcommand{\taylor}{{\text{Tay}}} 
\newcommand{\asympt}{{\text{Asy}}}  
\newcommand{\algo}{{\text{alg}}}  
\newcommand{\inter}{{\text{inter}}}  
%\newcommand{\He}{{{\dagger}}}

\newcommand{\lambdav}{\mbox{\boldmath$\lambda$}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\muv}{\mbox{\boldmath$\mu$}}
\newcommand{\omegav}{\mbox{\boldmath$\omega$}}
\newcommand{\sigmav}{\mbox{\boldmath$\sigma$}}

\newcommand{\re}[1]{(\ref{#1})}
\newcommand{\myse}{\IEEEyessubnumber} % setting subnumbering
\newcommand{\myses}{\myse\IEEEeqnarraynumspace} % setting subnumbering, shifted
